Peaking into the Black-box: Prediction Intervals Give Insight into Data-driven Quadrotor Model Reliability

Ensuring the reliability and validity of data-driven quadrotor model predictions is essential for their accepted and practical use. This is especially true for grey- and black-box models wherein the mapping of inputs to predictions is not transparent and subsequent reliability notoriously difficult to ascertain. Nonetheless, such techniques are frequently and successfully used to identify quadrotor models. Prediction intervals (PIs) may be employed to provide insight into the consistency and accuracy of model predictions. This paper estimates such PIs for polynomial and Artificial Neural Network (ANN) quadrotor aerodynamic models. Two existing ANN PI estimation techniques - the bootstrap method and the quality driven method - are validated numerically for quadrotor aerodynamic models using an existing high-fidelity quadrotor simulation. Quadrotor aerodynamic models are then identified on real quadrotor flight data to demonstrate their utility and explore their sensitivity to model interpolation and extrapolation. It is found that the ANN-based PIs widen considerably when extrapolating and remain constant, or shrink, when interpolating. While this behaviour also occurs for the polynomial PIs, it is of lower magnitude. The estimated PIs establish probabilistic bounds within which the quadrotor model outputs will likely lie, subject to modelling and measurement uncertainties that are reflected through the PI widths.

==> content/intro_full.tex <==

%==============================================================================================
% Introduction
%==============================================================================================
\section{Introduction}

\lettrine{D}{ata-driven} system identification techniques are often employed to develop models of highly non-linear systems, such as the quadrotor. These data-driven approaches to quadrotor model identification are convenient and attractive due to limited knowledge on analytical descriptions of the quadrotor \cite{Sun2018_GrayBox,hoffmann2007_QuadrotorAero,powers2013_AeroInfluence,Mahony2012_MAVS}. Subsequently, many quadrotor models have been successfully identified in literature using a plethora of system identification techniques \cite{Sun2018_GrayBox,Sun2018_IDQuadHS,Bansal2016,Mohajerin2018,bauersfeld2021neurobem}.

Of particular note are the high-speed grey-box quadrotor aerodynamic models identified by Sun et al. \cite{Sun2018_GrayBox} through polynomial step-wise regression. By exploiting knowledge on influential states of the system, informed choices on the candidate regressors are made. The term 'grey-box' stems from the fact that the physical meaning behind some of these regressors, and interactions therein, can be ambiguous. While the identified models of Sun et al. \cite{Sun2018_GrayBox} harbor desirable performance, the reliability of the models' predictions is not assessed in depth. Subsequently, even though the selected regressors are visible in the final model, the models occasionally produce unexpected predictions, particularly when noise is present in the system. 

Artificial neural networks (ANNs) are an increasingly popular choice by virtue of their generalizability \cite{Bansal2016} and aptitude for capturing unknown non-linearities \cite{Lu1998,Chen1990}. Consequently, they are employed to capture dynamics in unexplored and extreme regions of the flight envelope. Take, for instance, the use of ANNs to facilitate high-speed (i.e. up to $18$ $ms^{-1}$) quadrotor model identification by Bauersfeld et al. \cite{bauersfeld2021neurobem}. However, as a black-box modelling technique, it is ambiguous as to how exactly the ANN inputs interact to produce the model outputs. As such, evaluating the reliability and validity of the resultant ANN models is challenging and proves to be a significant barrier to their widespread use in the aerospace industry \cite{Schumann03onverification}. Although many ANN quadrotor models have been identified in literature with desirable performance (see, for example, \cite{bauersfeld2021neurobem,Mohajerin2018,Bansal2016}), none specify how reliable or valid these models are beyond assessing their performance with respect to some, typically unseen (i.e. validation), flight data sets. Good performance may be constrained to those data sets alone, and may lead to unpredictable model outputs for similar (e.g. noisy) inputs \cite{Khosravi2011_NN_Prediction_intervals}. Ensuring safety and reliability are paramount to the accepted use of autonomous quadrotors and thus this lack of model reliability measures for such black-box (and grey-box) modelling needs to be addressed. %Despite this, there is a distinct lack of methods in literature which assess the confidence and validity of identified ANN quadrotor models beyond evaluating their performance against a test/validation data-set. 

One way to describe the reliability of a model's prediction is through its confidence in that prediction. To this end, the associated prediction intervals (PIs) - the interval wherein a future observation will lie, with a given probability (i.e. confidence) - may be used as a proxy for reliability. For some grey-box system identification approaches, such as polynomial step-wise regression \cite{Klein2006_AircraftSysID}, there are valid analytical formulations for obtaining these PIs. However, due to the inherent obscurity behind black-box models, analytical formulations that maintain the validity of any estimated PIs are challenging, if not impossible, to derive. 

Consequently, some ANN literature \cite{Khosravi2011_NN_Prediction_intervals,KhosraviLUBE,pearce2018highquality,pearce2020uncertainty} propose various methods to estimate these prediction intervals, especially in the face of input uncertainties. One of the more straightforward and convenient approaches is known as the bootstrap method wherein an additional ANN is employed to estimate the PIs associated with the aggregate prediction of an existing ensemble of ANNs \cite{Khosravi2011_NN_Prediction_intervals}. This approach is particularly attractive as it may be applied to an already trained ensemble of ANNs without needing to retrain the underlying ensemble. In their review of popular ANN PI estimation techniques, Khosravi et al. \cite{Khosravi2011_NN_Prediction_intervals} found that the bootstrap approach did well to reflect uncertainty in the inputs. However, the bootstrap method often produces excessively wide PIs, which is undesirable. Instead, it is perhaps more lucrative to augment the training procedure in some way to ensure high-quality (i.e. valid, yet narrow) PIs. Accordingly, Pearce et al. \cite{pearce2018highquality} propose a quality-driven direct estimation of the PIs which incorporates common PI quality metrics directly in the cost function. This approach builds upon the lower upper bound estimation (LUBE) \cite{KhosraviLUBE} method, but is argued to produce higher quality, and valid, PIs \cite{pearce2018highquality}. These ANN PI estimation methods, or indeed any others, provide a clear utility in establishing model reliability but have yet to be applied to ANN quadrotor aerodynamic models.

Therefore, these methods are numerically validated for such models for the first time through an existing high-fidelity quadrotor simulation developed by Sun et al. \cite{Sun_ControlDoubleFailure,Sun2018_GrayBox}. Moreover, as the analytically derived prediction intervals for polynomial quadrotor aerodynamic models have also yet to be validated, these are also evaluated numerically. The subsequent results provide insight into the suitability and limitations of the all PI estimation methods and impose method-specific requirements on the uncertainty characteristics of the flight data for reliable PI estimates. 

% This paper continues with a brief introduction to the PI quality metrics and estimation methods for the polynomial, bootstrap, and direct methods in \cref{sec:PI}. Subsequently, the procedures for the numerical validation experiments, including a brief description of the simulation set-up used for data generation, are provided in \cref{subsubsec:procesdures_numerical_validation}. The numerical validation results themselves are then summarized and discussed in \cref{sec:PI_results}. Finally, \cref{sec:conclusion} concludes this paper alongside some recommendations for future work. 




%==============================================================================================
% EXTRA
%==============================================================================================


% Therefore, due to the promising results of both the bootstrap and quality-driven direct estimation methods, they are applied to quadrotor identification and PI estimation in this paper. PIs are only useful if they truly reflect the specified confidence behind making predictions. Consequently, the validity of the estimated PIs from these two methods are evaluated numerically for the first time using noisy data derived from an existing high-fidelity quadrotor simulation platform developed by Sun et al. \cite{Sun_ControlDoubleFailure}. This simulation is used to generate mock flight data under controlled conditions for two numerical validation experiments. While not as definitive as an analytical derivation, numerically corroborated PIs nonetheless lend support to their reliability and validity. Moreover, the polynomial prediction intervals, which are known to be reliable given their analytical foundations, are also identified for equivalent polynomial models to act as a benchmark during this numerical validation. 


% Subsequently, the most reliable ANN PI estimation method is elected for use with the ANN-based model identification. Therefore, the identified models (i.e. both polynomial and ANNs) in this paper are accompanied with reliable prediction intervals (PIs) which provide insight into the overall confidence of the model predictions. 


%Moreover, the PI coverage probability (PICP) and mean PI width (MPIW) are found to be reflective of the model validity, and prove to be useful PI metrics. 

% This is especially concerning for black-box models, such as the ANNs, for which the mapping of inputs to predictions is ambiguous and subsequent reliability notoriously difficult to ascertain. In an effort to address this, the use of model prediction intervals (PIs) to accompany model predictions is proposed. Such PIs provide insight into the confidence, and thus reliability, of the models' predictions. While there are analytical formulations for obtaining such valid PIs for polynomial models, there are only unproven PI estimation techniques for ANNs. Moreover, these have not been applied to, or even validated for, quadrotors.



% Indeed, some literature \cite{GEVREY2003249,SCARDI1999213} discusses methods for assessing input importance for ANNs in which parallels to input sensitivity analyses may be drawn. Some examples include the 'perturbation' method, wherein the change in model output accuracy is assessed by either removing or varying a given input variable \cite{GEVREY2003249}, or the 'input weight' method which associates the relative importance of a given (normalized) input with the corresponding connection weight \cite{GEVREY2003249}. However, these methods are typically aimed at determining essential variables to reduce input dimensionality, and therefore do not strictly evaluate how sensitive the ANNs are these inputs. Nonetheless, these methods may be employed to provide insight into which inputs the ANNs consider significant. Ensuring safety and reliability are paramount to the accepted use of autonomous quadrotors, especially for outdoor operations, and thus this lack of model validation needs to be addressed. 


% For example, Sun et al. \cite{Sun2018_GrayBox} identify high-speed polynomial models of a quadrotor through step-wise regression. By exploiting knowledge on influential states of the system, informed choices on the candidate regressors are made. However, what exactly some of these regressors and interactions therein entail physically may be ambiguous, hence the term 'gray-box'. Others instead prefer to employ black-box techniques, such as Artificial Neural Networks (ANN), to facilitate model identification and have been shown to improve upon quadrotor model accuracy \cite{Bansal2016,Bagherzadeh2018,Mohajerin2018,bauersfeld2021neurobem}. While such ANNs are powerful due to their generalizability \cite{Bansal2016} and aptitude for capturing unknown non-linearities \cite{Lu1998,Chen1990}, the mapping of inputs to predictions is ambiguous. 
%culminating in a 'gray-box' approach. Therefore, 


%An ANN model may produce accurate predictions for both the training and test set and thus may be considered a good model. However, such performance may be constrained to those data sets alone, and may deteriorate due to uncertainties in the inputs which ultimately culminate in erroneous predictions. This is undesirable as it may lead to unpredictable model outputs for similar inputs. 

==> content/method_full.tex <==
%==============================================================================================
% Validation methods for identified models -> Methodology
%==============================================================================================
\section{Methods}\label{sec:method}

\subsection{Prediction intervals}\label{subsec:prediction_intervals}
Although regression aims to approximate a certain target variable given a set of predictors, measurements of these targets are, in practical applications, often contaminated with bias and noise. Moreover, further uncertainties and errors arise from modelling misspecification. Both sources of uncertainty induce a variation in model predictions, which may be modelled through \cref{eq:total_variance} \cite{Khosravi2011_NN_Prediction_intervals}. Here, $\boldsymbol{\sigma}_{\hat{\boldsymbol{\epsilon}}}^{2}$ encompasses the uncertainty associated with the predictions and measurement and $\boldsymbol{\sigma}_{\hat{\mathbf{y}}}^{2}$ denotes the variance due to modelling misspecification. 

\begin{equation}\label{eq:total_variance}
    \boldsymbol{\sigma}^{2} = \boldsymbol{\sigma}_{\hat{\mathbf{y}}}^{2} + \boldsymbol{\sigma}_{\hat{\boldsymbol{\epsilon}}}^{2}
\end{equation}

% $\boldsymbol{\sigma}^{2}$ gives the variance associated with the total model predictions and may therefore be used to construct the prediction intervals (PIs) based on a given confidence level $1-\alpha$. In this paper, the PI is defined as the interval in which a future observation will lie, provided that it has previously been observed, up to a specified confidence level. Note that, by definition, the PIs enclose the confidence interval (CI), which only accounts for $\boldsymbol{\sigma}_{\hat{\mathbf{y}}}^{2}$. The corresponding PI bounds, for a given target value, $y_{i}$, and associated total variance, $\sigma _{i}$, can be obtained through \cref{eq:PI_bounds}. In \cref{eq:PI_bounds}, $t^{1-\alpha/2}_{N-2}$ gives two sided test statistic for the chosen confidence level, $1 - \alpha$, and $n$ gives the number of observations. Typically, $n=1$ when making (single) predictions.  
$\boldsymbol{\sigma}^{2}$ gives the variance associated with the total model predictions and may therefore be used to construct the prediction intervals (PIs) based on a given confidence level $1-\alpha$. The corresponding PI bounds, for a given target value, $y_{i}$, and associated total variance, $\sigma _{i}$, can be obtained through \cref{eq:PI_bounds}. In \cref{eq:PI_bounds}, $t^{1-\alpha/2}_{N-2}$ gives two sided test statistic for the chosen confidence level, $1 - \alpha$, and $n$ gives the number of observations. 

\begin{equation}\label{eq:PI_bounds}
\begin{array}{ccc}
    y_{i}^{L} = \hat{y}_{i} - t^{1-\alpha/2}_{N-2}\frac{\sigma _{i}}{\sqrt{n}}, & & y_{i}^{U} = \hat{y}_{i} +  t^{1-\alpha/2}_{N-2}\frac{\sigma _{i}}{\sqrt{n}}
\end{array}
\end{equation}

% Two metrics are typically employed to evaluate the quality of the PIs: the Coverage Probability (PICP) and the Mean Prediction Interval Width (MPIW) \cite{Khosravi2011_NN_Prediction_intervals,pearce2018highquality}. The PICP is defined in \cref{eq:PICP}, where $N$ denotes the number of test data points, and $c_{i}$ describes if the target value is contained within the defined bounds of the PI (where $L_{i}$ = lower bound, $U_{i}$ = upper bound) for a given confidence level. Therefore, the PICP may be used to verify whether the desired confidence level is achieved. For example, PIs designed to capture the target value 95\% of the time are expected to maintain a $PICP \ge 95\%$. %While the PICP is useful for evaluating the validity of the PIs, it does not itself describe how practical the PIs are since infinitely large PIs also satisfy the PICP requirement. 

The PI coverage probability (PICP) is often used to access the quality of a PI by verifying if the desired confidence level is reached \cite{Khosravi2011_NN_Prediction_intervals,pearce2018highquality} and is defined in \cref{eq:PICP}. $N$ denotes the number of test data points, and $c_{i}$ describes if the target value is contained within the defined bounds of the PI (where $L_{i}$ = lower bound, $U_{i}$ = upper bound) for a given confidence level. 

\begin{equation}\label{eq:PICP}
\begin{array}{cc}
     &  PICP = \frac{1}{N}\sum_{i=1}^{N}c_{i} \\
    \text{where} & \\
     &  c_{i} = \left \{ \begin{array}{ll} 1, & y_{i} \in [L_{i}, U_{i}] \\ 0, & \text{otherwise}\end{array} \right.
\end{array}
\end{equation}

% Complimentary to the PICP, the MPIW is often used to parameterize the width of the PIs and is typically normalized with respect to the range of the target data. The normalized MPIW is defined in \cref{eq:MIPW}. Both the PICP and the MPIW should be used in tandem to describe the overall PI quality, seeing as the deficiencies of one metric are perfectly accommodated by the other. Therefore, a 'high-quality' PI is one which satisfies the PICP requirement while being as narrow as possible in terms of the (normalized) MPIW. 

Complimentary to the PICP, the MPIW is often used to parameterize the width of the PIs and is typically normalized with respect to the range of the target data. The normalized MPIW is defined in \cref{eq:MIPW}. Both the PICP and the MPIW should be used in tandem to describe the overall PI quality, seeing as the deficiencies of one metric are perfectly accommodated by the other.


\begin{equation}\label{eq:MIPW}
    MIPW = \frac{1}{N}\sum_{i=1}^{N}{(U_{i} - L_{i})}
\end{equation} 

\subsubsection{Polynomial}
Conveniently, for polynomial models, the total variance associated with a prediction may calculated through \cref{eq:OLS_sigma} under the assumptions that the measurement error term, $\epsilon$, is zero-mean, independent and identically distributed. In \cref{eq:OLS_sigma}, $\mathbf{x_{0}}$ denotes the input data for which predictions should be made (i.e. to predict $y_{0}$), $\mathbf{X}$ represents the regressor matrix used for training the model, $\mathbf{I}$ gives the identity matrix and $\sigma_{e}^{2}$ may be approximated through \cref{eq:sigma_est}.

% Here, we assume weights are Gaussian \cref{eq:OLS_sigma}

\begin{equation}\label{eq:OLS_sigma}
    \hat{\sigma}_{0}^{2} = \sigma_{e}^{2} \left ( \mathbf{I} + \mathbf{x}_{0} \left ( \mathbf{X}^{T} \mathbf{X} \right )^{-1} \mathbf{x}_{0}^{T} \right )
\end{equation}

\begin{equation}\label{eq:sigma_est}
    \hat{\sigma}_{e}^{2} = \frac{1}{N_{t}-2}\sum_{i=1}^{N}{\hat{e}_{i}^{2}}
\end{equation}

In \cref{eq:sigma_est}, $N_{t}$ represents the number of samples used for training and $\hat{e}_{i} = y_{i} - \hat{y}_{i}$ denotes the residual error. The computed $\hat{\sigma} _{0}$ may then be inputted into \cref{eq:PI_bounds} to obtain the lower and upper bounds of the PI. 



\subsubsection{ANN: Bootstrap}

The bootstrap method exploits the inherent stochasticity of the ANN training process and can be applied to an already trained ensemble of ANNs. The spread (i.e. variance) of predictions across an ensemble of ANN models, initialized with distinct weights and trained on different subsets of the training data set, gives an approximation of the model misspecification uncertainty \cite{Khosravi2011_NN_Prediction_intervals,pearce2018highquality}. This variance may be constructed through \cref{eq:bootstrap_sig_hat} \cite{Heskes97practicalconfidence,Khosravi2011_NN_Prediction_intervals}, where $B$ gives the number of ANN models $\hat{y}_{i}$ denotes the ensemble average predicted value of the target. 

\begin{equation}\label{eq:bootstrap_sig_hat}
    \hat{\sigma}_{y_{i}}^{2} = \frac{1}{B-1}\sum_{j=1}^{B}{\left ( \hat{y}_{i}^{j} - \hat{y}_{i} \right )^{2}}
\end{equation}

The variance due to the measurement errors, $\sigma_{\epsilon_{i}}$, is typically unknown and cannot easily be inferred from the ensemble of ANN models. Instead, an additional ANN (hereafter known as the $\sigma_{\epsilon_{i}}^{2}$-predictor ANN) may be used to (implicitly) estimate this variance using a data set that is distinct from that used for training \cite{Heskes97practicalconfidence,Khosravi2011_NN_Prediction_intervals}. Using the residuals between the model predictions and the target data, a new data set, $D_{r} = \{ x_{i}, r_{i}^{2} \}_{i=1}^{m}$, may be constructed linking the inputs, $x_{i}$, to the variance residuals, $r_{i}^{2}$, defined in \cref{eq:bootstrap_variance_residuals} \cite{Khosravi2011_NN_Prediction_intervals}. %Note the 'max' operator is used here since the variance should be greater than zero.

% Using the (trained) ensemble of ANNs, predictions can be made for this unseen data set for which the target values are known and subsequent squared errors taken through \cref{eq:squared_errors_Bootstrap}. Since the variance due to the model uncertainty has been approximated through the variance in ANN predictions in the ensemble (i.e. \cref{eq:bootstrap_sig_hat}), the remaining variance in the squared errors, $e_{i}^{2}$, is assumed to be the variance of the measurement noise errors, $\sigma_{\epsilon_{i}}^{2}$ \cite{Heskes97practicalconfidence}. Therefore, a new data set, $D_{r} = \{ x_{i}, r_{i}^{2} \}_{i=1}^{m}$, may be constructed linking the inputs, $x_{i}$, to the variance residuals, $r_{i}^{2}$, defined in \cref{eq:bootstrap_variance_residuals}. Note the 'max' operator is used here since the variance should be greater than zero.

% \begin{equation}\label{eq:squared_errors_Bootstrap}
%     e_{i}^{2} = (y_{m,i}- \hat{y}_{i})^{2}
% \end{equation}

\begin{equation}\label{eq:bootstrap_variance_residuals}
    r_{i}^{2} = \max \left ( \left ( y_{m,i} - \hat{y}_{i})^{2} - \hat{\sigma}_{y_{i}}^{2} \right ), 0 \right )
\end{equation}
% =============================================================================
% NOTE: 
% - It is extremely challenging, if not impossible, to obtain a dataset with a variance of targets per measurement sample.
% - Hence, we approximate this through \cref{eq:bootstrap_variance_residuals}, where we take the remaining error between targets and predictions, while accounting for the current model uncertainty. 
% - The result of this is that the estimated PIs are conservative (since sigma < r is penalized heavily in the loss function, J), and should at least encompass variation due to model uncertainty (i.e. the PIs). 
% =============================================================================



% The $\sigma_{\epsilon_{i}}^{2}$-predictor ANN may then be used to implicitly approximate $\sigma_{\epsilon_{i}}^{2}$ by minimizing the cost function defined in \cref{eq:bootstrap_cost_function} \cite{Khosravi2011_NN_Prediction_intervals}. This cost function is obtained by taking the natural logarithm of the normal distribution of $\epsilon$ and thus ensures that the $\sigma_{\epsilon_{i}}^{2}$-predictor ANN produces variances which conform this normal distribution \cite{Khosravi2011_NN_Prediction_intervals}. The practical implementation of this cost function involves setting $r_{i}^{2}$ as the target values (i.e. $r_{i}^{2} \to y_{i}$) and $\sigma_{\epsilon_{i}}^{2}$ as the ANN predicted values (i.e. $\sigma_{\epsilon_{i}}^{2} \to \hat{y}_{i}$). 

The $\sigma_{\epsilon_{i}}^{2}$-predictor ANN may then be used to implicitly approximate $\sigma_{\epsilon_{i}}^{2}$ by minimizing the cost function defined in \cref{eq:bootstrap_cost_function} \cite{Khosravi2011_NN_Prediction_intervals}. Note that this cost function is derived under the assumption of Gaussian errors. %This cost function is obtained by taking the natural logarithm of the normal distribution of $\epsilon$ and thus ensures that the $\sigma_{\epsilon_{i}}^{2}$-predictor ANN produces variances which conform this normal distribution \cite{Khosravi2011_NN_Prediction_intervals}. The practical implementation of this cost function involves setting $r_{i}^{2}$ as the target values (i.e. $r_{i}^{2} \to y_{i}$) and $\sigma_{\epsilon_{i}}^{2}$ as the ANN predicted values (i.e. $\sigma_{\epsilon_{i}}^{2} \to \hat{y}_{i}$). 

\begin{equation}\label{eq:bootstrap_cost_function}
    J = \frac{1}{2}\sum_{i=1}^{m}{\left [ \ln{(\sigma_{\epsilon_{i}}^{2})} + \frac{r_{i}^{2}}{\sigma_{\epsilon_{i}}^{2}} \right ]}
\end{equation}



% % Since the $\sigma_{\epsilon_{i}}^{2}$-predictor ANN is separate from the main model collection of ANNs, it is easily added to existing model ensembles to approximate the PIs, and by extension the confidence, involved in the model aggregate predictions. 

% As with the polynomial PIs, \cref{eq:PI_bounds} may be used to construct the lower and upper PI bounds using the complete estimated model prediction variance, $\hat{\sigma}_{i} = \hat{\sigma}_{y_{i}} + \hat{\sigma}_{\epsilon_{i}}$. %However, it is important that the inputs used to construct $D_{r}$ are distinct from those used for training and validating the network ensembles. Hence, a slight modification of the training data sets may also be necessary.  

% Intuitively, more models used in the ensembles leads to more reliable estimates for the model uncertainty. Consequently, some literature, such as \cite{davison_hinkley_1997,efron1994introduction}, advocate for the use of hundreds to thousands of ANN models. This rather problematic given that training such an extensive collection of models demands significant computational resources and casts doubt on the practical application of the bootstrap method for quadrotor modelling. However, both \cite{Khosravi2011_NN_Prediction_intervals,pearce2018highquality} found that as few as 5-10 ANN models are sufficient for producing reliable prediction intervals. Although, it should be highlighted that the minimum number of ANNs in an ensemble is dependent on the modelling task at hand, and may increase, or decrease, depending on the complexity of employed ANNs and the modelling task itself. 

% While the bootstrap method may not result in the best quality PIs, often with excessively wide PIs, it is simple to implement and may be applied directly to existing ANNs without interfering with the training process \cite{Khosravi2011_NN_Prediction_intervals}. For quadrotor applications, a more conservative estimate (i.e. wider MPIWs) may be argued to be desirable as it promotes greater caution in predictions. Moreover, the bootstrap method intuitively reflects uncertainties in the inputs (i.e. higher uncertainties results in wider PIs) \cite{Khosravi2011_NN_Prediction_intervals}. %Moreover, the bootstrap method is computationally efficient when making predictions\footnote{Note that this method is, however, computationally demanding during training. This complexity also scales with the number of necessary model ensembles for reliable predictions.} compared to other ANN PI estimation methods and it is found to intuitively reflect uncertainties in the inputs (i.e. higher uncertainties results in wider PIs) \cite{Khosravi2011_NN_Prediction_intervals}. 



\subsubsection{ANN: Quality driven}
Instead of estimating the PIs after-the-fact, another approach is to estimate them directly \cite{KhosraviLUBE} while considering the PI quality metrics (i.e. $PICP$ and $MPIW$). Such an approach is outlined in the recent work of Pearce et al. \cite{pearce2018highquality} wherein a 'quality-driven' (QD) loss function incorporating both the $PICP$ and $MPIW$ is used to train an ensemble of FNNs. The output of each network are the upper and lower bounds of the PI associated with a prediction. The QD loss function is described in \cref{eq:QD}. $MPIW_{C}$ denotes the (normalized) mean widths of the PIs, provided that the target point is contained within the PI bounds for that sample. $N$ is the batch size used for training. 

\begin{equation}\label{eq:QD}
    QD = MPIW_{C} + N\lambda\max{(0, (1 -\alpha) - PICP_{s})}^{2}
\end{equation}

$PICP_{s}$ represents the 'soft' PICP, defined in \cref{eq:PICP_s} where $\sigma(\cdot)$ denotes the sigmoid function and $s$ is some softening factor. Pearce et al. \cite{pearce2018highquality} found that $s=160$ consistently produces acceptable results across multiple different regression tasks. A 'softening' of the $PICP$ is encouraged to mitigate the non-linearity of the second term in \cref{eq:QD} for compatibility with the optimizers of existing neural network library implementations (e.g. \texttt{tensorflow}). 

\begin{equation}\label{eq:PICP_s}
    PICP_{s} = \frac{1}{N}\sum_{i=1}^{N}{\sigma(s(y_{i} - \hat{y}_{L,i}))\cdot\sigma(s(\hat{y}_{i,U} - y_{i}))}
\end{equation}


\subsection{Model identification}\label{subsec:system_identification}
For all modelling techniques, individual aerodynamic models are identified for the forces and moments of each of the axes (i.e. 6 models total, per technique). 

Polynomial aerodynamic models are identified through step-wise regression \cite{Klein2006_AircraftSysID} following the same procedure as outlined by Sun et al. \cite{Sun2018_GrayBox} for their grey-box models. In consultation with the authors of \cite{Sun2018_GrayBox}, the rotor speeds are also incorporated in the candidate regressors for improved performance.

The architectures of the ANN models for both PI estimation techniques is identical with only method-specific differences. Inspired by the ANNs of \cite{Bansal2016}, all ANN models used here are composed of an ensemble of 10 dense feed-forward neural networks, each with an input layer, a hidden layer with 20 neurons, and an output layer. ReLU and a linear function constitute the hidden layer and output layer activation functions respectively and ADAM is used as the optimizer. The mean-squared-error and QD cost functions are employed for the bootstrap and quality-driven methods respectively. All ANNs are trained for 50 epochs. For the bootstrap method, an additional FNN with identical structure to the base ANNs is used, with the exception of 25 hidden neurons and a modified cost function given by \cref{eq:bootstrap_cost_function}.


\subsection{Data generation}\label{subsec:data_generation}

An existing high-fidelity quadrotor simulation, developed by Sun et al. \cite{Sun_ControlDoubleFailure}, is used to generate mock-flight data for quadrotor model identification and PI numerical validation under consistent conditions. In the simulation, users can specify positional and yaw commands. These are used to generate a collection of simulated flight trajectories for model identification (training set) and numerical validation (validation set). All reference signals are either step-like pulses or sinusoidal in nature, with varying amplitude and frequency. The training set consists of both decoupled and coupled force and moment manoeuvres (e.g. decoupled: sinusoid along x-axis for pitching moment and force along x; coupled: sinusoid along all axes). The validation set only consists of coupled manoeuvres, distinct from those seen during training (e.g. different couplings or reference signals).

As the simulation relies on a non-linear controller, the flight data is initially generated noise-free to avoid the non-Gaussian transformation of uncertainty. "Noise", sampled from a Gaussian distribution, is then added to each of the model inputs and targets to simulate uncertainty. For numerical validation, the identified models are tasked with making predictions on the 1000, noise contaminated, realizations of the validation set. The subsequent spread in model predictions and true targets is observed, and the ability of the PIs to contain these evaluated for each run. 



% =========================================================================================================
% =========================================================================================================
% =========================================================================================================
% =========================================================================================================
